Improving Object Detection, Multi-object Tracking, and Re-Identification for Disaster Response Drones

We aim to detect and identify multiple objects using multiple cameras and computer vision for disaster response drones. The major challenges are taming detection errors, resolving ID switching and fragmentation, adapting to multi-scale features and multiple views with global camera motion. Two simple approaches are proposed to solve these issues. One is a fast multi-camera system that added a tracklet association, and the other is incorporating a high-performance detector and tracker to resolve restrictions. (...) The accuracy of our first approach (85.71%) is slightly improved compared to our baseline, FairMOT (85.44%) in the validation dataset. In the final results calculated based on L2-norm error, the baseline was 48.1, while the proposed model combination was 34.9, which is a great reduction of error by a margin of 27.4%. In the second approach, although DeepSORT only processes a quarter of all frames due to hardware and time limitations, our model with DeepSORT (42.9%) outperforms FairMOT (71.4%) in terms of recall. Both of our models ranked second and third place in the `AI Grand Challenge' organized by the Korean Ministry of Science and ICT in 2020 and 2021, respectively. The source codes are publicly available at these URLs (github.com/mlvlab/drone_ai_challenge, github.com/mlvlab/Drone_Task1, github.com/mlvlab/Rony2_task3, github.com/mlvlab/Drone_task4).

==> abstract.tex <==
We aim to detect and identify multiple objects using multiple cameras and computer vision for disaster response drones. The major challenges are taming detection errors, resolving ID switching and fragmentation, adapting to multi-scale features and multiple views with global camera motion.
Two simple approaches are proposed to solve these issues. One is a fast multi-camera system that added a tracklet association, and the other is incorporating a high-performance detector and tracker to resolve restrictions.

The first approach generally improves tracking accuracy in crowded scenes. The expected problems are ID fragmentation caused by fast-moving people or people going out of the scene and occlusions.
Fast-processing models are needed to handle the tracking and re-identification of many fast-moving people. OSNet is added to FairMOT to extract better representational feature vectors for associating persons detected from multiple drone cameras. The second approach focuses on real-world applications where camera movements are irregular and has limited hardware resources like a simulation of rescuing people in a kind of disaster situation. To get higher-quality tracking information in such circumstances, we focus on enhancing object detection performance by combining YOLOv5 and DeepSORT, and the post-processing after the re-ID block.

The accuracy of our first approach (85.71\%) is slightly improved compared to our baseline, FairMOT (85.44\%) in the validation dataset. In the final results calculated based on L2-norm error, the baseline was 48.1, while the proposed model combination was 34.9, which is a great reduction of error by a margin of 27.4\%. In the second approach, although DeepSORT only processes a quarter of all frames due to hardware and time limitations, our model with DeepSORT (42.9\%) outperforms FairMOT (71.4\%) in terms of recall.

Both of our models ranked second and third place in the ``AI Grand Challenge'' organized by the Korean Ministry of Science and ICT in 2020 and 2021, respectively.
The source codes are publicly available at these URLs
\footnote{https://github.com/mlvlab/drone\_ai\_challenge}
\footnote{https://github.com/mlvlab/Drone\_Task1}
\footnote{https://github.com/mlvlab/Rony2\_task3}
\footnote{https://github.com/mlvlab/Drone\_task4}
.

==> acknowledgement.tex <==
This work was supported in part by the Institute of Information and Communications Technology Planning and Evaluation (IITP) Grants by the Korean Government through the Ministry of Science and ICT (MSIT) (Development of Integrated Cognitive Drone AI for Disaster/Emergency Situations) under Grant 2021-0-00025.
